Noise-Tolerant Coreset-Based Class Incremental Continual Learning

Many applications of computer vision require the ability to adapt to novel data distributions after deployment. Adaptation requires algorithms capable of continual learning (CL). Continual learners must be plastic to adapt to novel tasks while minimizing forgetting of previous tasks.However, CL opens up avenues for noise to enter the training pipeline and disrupt the CL. This work focuses on label noise and instance noise in the context of class-incremental learning (CIL), where new classes are added to a classifier over time, and there is no access to external data from past classes. We aim to understand the sensitivity of CL methods that work by replaying items from a memory constructed using the idea of Coresets. We derive a new bound for the robustness of such a method to uncorrelated instance noise under a general additive noise threat model, revealing several insights. Putting the theory into practice, we create two continual learning algorithms to construct noise-tolerant replay buffers. We empirically compare the effectiveness of prior memory-based continual learners and the proposed algorithms under label and uncorrelated instance noise on five diverse datasets. We show that existing memory-based CL are not robust whereas the proposed methods exhibit significant improvements in maximizing classification accuracy and minimizing forgetting in the noisy CIL setting.

==> sec/3_problem.tex <==
\section{Problem Definition}
\label{sec:problem}

CL addresses the challenge of learning from a dynamic stream of data that exhibit distribution shifts while maintaining previous knowledge. We can formalize the CL problem as follows. Let $\{(x_t, y_t)\}_{t=1}^T$ be a sequence of input-output pairs (data and labels in the supervised case), where $x_t \in \mathcal{X}$ and $y_t \in \mathcal{Y}$. The goal is to learn a function $f_\theta: \mathcal{X} \rightarrow \mathcal{Y}$ that minimizes:

\begin{equation}
    \min_\theta \mathbb{E}_{(x,y) \sim p_t(x,y)} [\mathcal{L}(f_\theta(x), y)]
\end{equation}

where $p_t(x,y)$ is the joint distribution at time $t$, and $\mathcal{L}$ is a loss function. In most CL settings,  the learning process is divided into sequences of $K$ tasks with associated probabilities $p_k(x,y)$. We can express the CL objective as:

\begin{equation}
    \min_\theta \sum_{k=1}^K \mathbb{E}_{(x,y) \sim p_k(x,y)} [\mathcal{L}(f_\theta(x), y)]
\end{equation}
This objective is subject to a constraint that performance on previous tasks does not significantly degrade:
\begin{equation}
    \mathbb{E}_{(x,y) \sim p_j(x,y)} [\mathcal{L}(f_\theta(x), y)] \leq \epsilon_j, \quad \forall j < k
\end{equation}
where $\epsilon_j$ represents acceptable performance degradation on previous tasks.


==> sec/4_method.tex <==
\section{Methodology}
\label{sec:methods}
We introduce two strategies for continual learning: Continual CRUST and Continual CosineCRUST, both focusing on selecting representative data subsets (coresets) for maintaining performance across evolving tasks.

\subsection{Coresets for Robust Training (CRUST)}
\label{sec:crust}

CRUST \cite{mirzasoleiman2020coresets} was introduced as a method for training of neural networks robust to noisy labels in the static learning setting. It is a coreset selection technique designed to improve generalization of models by selecting clean data samples from noisy training datasets. CRUST minimizes the influence of noisy labels by utilizing the Jacobian of the neural network to identify the most relevant samples for ongoing training, reducing training data size without compromising accuracy. Recent findings show that in the Jacobian matrix, a few singular values are quite large, while most others are small. The Jacobian spectrum can be divided into two parts: the Information space, which includes the large singular values, and the Nuisance space, made up of the small singular values \cite{oymak2020toward}. For complementary subspaces $S_{-}$ and $S_{+} \subset \mathbb{R}^n$ and for unit norm vectors $v \in S_{+}$ and $w \in S_{-}$ and scalars $0 \leq \gamma \ll \alpha \leq \beta$, we have:

$$\alpha \leq \|\mathcal{J}^T (W, X)v\|_2 \leq \beta \ \ \text{and } \ \ \|\mathcal{J}^T(W, X)w\|_2 \leq \gamma$$

Other studies \cite{oymak2020toward, li2020gradient} have found that learning in the small Information space is typically fast and generalizes to new data, but learning in the large Nuisance space is slow and leads to overfitting. How well a model generalizes to new data depends on how closely the true label ($y$) and the residual between the prediction and true label ($r=f(x) - y$) match the Information space. When there is a strong match, the model improves quickly during backpropagation. By focusing on the most informative clean data points, the model learns the underlying patterns in the data rather than memorizing noisy labels. For clean data samples, the label and the residual often fall in the Information space. For noisy data samples, they fall in the Nuisance space. CRUST leverages this idea to choose clean and highly discriminative data points.
\subsubsection{Theoretical Guarantees}
% (Restate theory from original CRUST paper
% Introduce extension to noisy data - Include proof sketch; point to full proof in the supplemental materials)

CRUST \cite{mirzasoleiman2020coresets} aims to select a representative subset of k diverse data points with clean labels that span the information space $\mathcal{I}$. This subset is chosen to have an approximately low-rank Jacobian matrix. There are two key principles considered by CRUST:

\begin{enumerate}
    \item [1.] CRUST utilizes the fact that important information in the dataset often lies in a low-dimensional space, facilitating efficient learning and better generalization.
    \item [2.] The method takes advantage of the observation that data points with clean labels tend to have similar gradients, clustering together in the gradient space.
\end{enumerate}

Let $V$ denote the complete dataset. The selection of $k$ data points for the coreset $S$ is defined by the following optimization problem:
\begin{equation}
S^* (W) \in \arg \min {S \subset V} \sum{i \in V} \min_{j \in S} d_{ij}(W) \ \ , \ |S| \leq k
\label{eq:optimization}
\end{equation}

where $d_{ij}(W) = \|\nabla \mathcal{L} (W, x_i) - \nabla \mathcal{L} (W, x_j)\|_2$ is the pairwise dissimilarity between gradients of data points $i$ from $V$ and $j$ from $S$. Solving this optimization does not yield the \textit{optimal} solution for the rank-$k$ approximation of the Jacobian, but the selected data points offer a reasonable approximation of the Jacobian derived from clean samples. 

An important consideration is that this strategy initially requires backpropagation on the entire dataset to compute the distances $d_{ij}$, which can be computationally intensive. Prior research \cite{katharopoulos2018not} has demonstrated that for neural networks, the variation in gradient norms is predominantly captured by the gradient of the loss with respect to the input of the last layer. Leveraging this insight significantly enhances the efficiency of the strategy. The approach can be made more numerically efficient by reformulating Equation \eqref{eq:optimization} as a submodular maximization problem:
\begin{equation}
    S^* \in \arg \max _{S \subset V \ , |S|\leq k} F(S, W)
    \label{maximizationproblem}
\end{equation}
where $F(S,W) = \sum_{i \in V} \max_{j \in S} d_0 - d'_{ij}(W)$ with $d_0$ to be a constant satisfying $d_0 \geq d_{ij}(W)$, for all $i, j \in V$.

% A set function $F: 2^V \rightarrow \mathbb{R}^+$ is submodular if for any $S \subset T \subset V$ and $e \in V \setminus T$:

% \begin{equation}
% F(S \cup \{e\}) - F(S) \geq F(T \cup \{e\}) - F(T)
% \end{equation}

To optimize Equation \eqref{maximizationproblem}, a greedy algorithm with complexity $\mathcal{O} (nk)$ is employed. It initializes with an empty set $S_0 = \varnothing$ and at each iteration $t$, selects an element $e \in V$ that maximizes the marginal utility $F(e|S_t) = F(S_t \cup \{e\}) - F(S_t)$:

\begin{equation}
S_t = S_{t-1} \cup \{\arg \max_{e \in V} F(e | S_{t-1})\}
\end{equation}

% This greedy approach provides an efficient method for approximating the optimal solution to the submodular maximization problem with a computation complexity $\mathcal{O} (nk)$. 

CRUST provides guarantees that for a small fraction $\rho$ of noisy labels in the coresets, deep networks do not overfit the noisy labels:

\begin{theorem}\label{thm:crust_convergence} (\textbf{Robustness to Label Flipping}) \cite{mirzasoleiman2020coresets}
    Assume that gradient descent is applied to train a neural network with mean-squared error loss on a dataset that contains clean and noisy labels. Suppose that the Jacobian of the network is $L$-smooth. Assume that the dataset has a label margin of $\delta$ and coresets found by CRUST contain a fraction of $\rho < \frac{\delta}{8}$ noisy labels. If the coresets approximate the Jacobian matrix by an error of at most $\epsilon \leq \mathcal{O} (\frac{\delta \alpha^2}{k \beta \log (\sqrt{k} / \rho)})$, where $\alpha = \sqrt{r_{min}} \sigma_{min} (\mathcal{J}(W, X_S)))$, $\beta = \|\mathcal{J} (W, X)\| + \epsilon$, then for $L \leq \frac{\alpha \beta}{L \sqrt{2 k}}$ and learning rate $\eta = \frac{1}{2 \beta^2}$, after $\tau \geq \mathcal{O} (\frac{1}{\eta \alpha^2} \log (\frac{\sqrt{n}}{\rho}))$ iterations the network classifies all the selected elements correctly.
\end{theorem}

We extend Theorem \ref{thm:crust_convergence} to encompass types of noise beyond label corruption, including Gaussian noise, salt and pepper noise, and other common stochastic perturbations on the data. A full proof of the theorem is included in the supplemental materials:

\begin{theorem} (\textbf{Robustness to Data Perturbations})\label{thm:random_noise}\\
Assume similar properties as Theorem \ref{thm:crust_convergence} but let $\delta$ be the part of the data we perturb: the proposed coresets approximate the Jacobian matrix error of at most $\epsilon \leq \mathcal{O}(\frac{\delta \alpha^2}{k \beta \log (\delta)})$ ($k$ is the size of the coresets from $n$ data points) where $\alpha = \sqrt{r_{min}} \sigma_{min} (\mathcal{J}(W, X_S)) - E_{min}$ and $\beta = \|\mathcal{J}(W, X_S)\|_2 + \epsilon + E_{max}$.  For $L \leq \frac{\alpha \beta}{L \sqrt{2 k}}$ and step size $\eta = \frac{1}{2 \beta^2}$ then after $T \geq \mathcal{O}(\frac{1}{\eta (\frac{\alpha}{2} +  E_{av}\alpha +  E \alpha -  \eta E_{av} \frac{\beta^3}{2} - \eta E \frac{\beta}{3})} \log \frac{\|r_0\|_2}{\nu})$ iterations, the network classifies all the selected elements correctly. (E values are errors coming from the perturbation)
\end{theorem}

% This extended theorem provides a comprehensive framework for understanding the robustness of our approach in the presence of diverse data perturbations. It demonstrates the method's effectiveness against various forms of data corruption, enhancing its applicability in real-world scenarios where noise extends beyond label errors.
Importantly, the provable guarantees from both theorems extend the practical applications of our method, providing confidence in the method's performance across a wide range of real-world data conditions. Data often contains various types of noise, and our approach's demonstrated robustness against these diverse noise types makes it particularly valuable for practical implementations.

\subsection{CosineCRUST}
% Discuss motivation behind cosine-crust
% Two major components: 
% cosine-distance 
% clustering + filtering out weak clusters

%Building upon insights from CRUST, we observe that data points with clean labels tend to have gradients that cluster closely together. This clustering behavior provides information for identifying and selecting representative data points. 
We introduce a modification of CRUST based on cosine distance. Cosine distance is a well-established metric that quantifies directional similarity between vectors, regardless of their magnitude:
\begin{equation}
\text{cosine\_distance}(a, b) = 1 - \frac{a \cdot b}{\|a\| \|b\|}
\end{equation}

where $a$ and $b$ are vectors, $\cdot$ denotes the dot product, and $\|\cdot\|$ represents the vector norm. %This metric is particularly suited for our purpose because:

% \begin{enumerate}
%     \item It measures how similar the directions of gradients are, helping us find data points that behave alike.
%     \item It ignores the magnitude of gradients, focusing only on their direction.
%     \item It provides a clear and interpretable measure, with values ranging from 0 (perfectly aligned) to 2 (oppositely aligned).
% \end{enumerate}

By incorporating cosine distance into our selection criteria, we hypothesize that we can more accurately identify clusters of data points with similar gradient behavior, improving the quality of the selected subset for CL tasks. Furthermore, instead of solving a single submodular optimization problem as is done in CRUST, we cluster data based on cosine similarity (using spectral clustering), filter out small clusters, which we hypothesize are noisy samples, and solve the submodular optimization within each cluster to form our final coreset. %, so that the selected data points cover the total dataset.

\subsection{Extension to Class-Incremental Continual Learning}
CRUST and CosineCRUST are designed for static ML problems but can be extended to build replay buffers for a memory-based continual learner. The ability to select small coresets that contain essential information about a given dataset allows for efficient knowledge preservation and transfer across different learning phases, mitigating catastrophic forgetting and enhancing model adaptability.

% Present algorithm for using Cosine-CRUST in the class-incremental setting
% As shown in Algorithm~\ref{alg:cosineCRUST}, we train a neural network for the current experience (which contains all information available at time $t$), comprising the full dataset for the current task and past experiences data stored in the coreset-driven replay buffer. The model learns patterns from the data, allowing us to extract valuable information from the gradients, which reflect the learned representations within the current task dataset.

For each experience, our model undergoes a two-phase training process spanning $n$ epochs (Algorithm~\ref{alg:cosineCRUST}). In the initial phase, lasting $m$ epochs ($m < n$), we train using the full dataset for classes in the current task set and the coresets for the classes from past experiences with class imbalanced handled via a weighted loss function or upsampling of past data. The subsequent phase, from epoch $m+1$ to $n$, focuses exclusively on training the neural network using coresets for both current and past classes, employing the cross-entropy loss. The gradients of the loss function with respect to the input of the last layer ($L-1$) are extracted for a full pass through the data. Based on the results on the cosince distance of the gradients, $k$ clusters are formed. Clusters containing a small number of samples are indicative of noisy data points, so $p<k$ clusters are used to select samples for the coreset ($p$ is determined based on a threshold on cluster size). Submodular optimization is applied to each cluster and samples for the coreset are drawn proportional to the cluster size. When the gradients are well-behaved, we hypothesize that the filtering of likely noisy samples and optimization based on diverse clusters (instead of global optimization) may lead to improved performance on the downstream tasks.

\begin{algorithm}
\caption{Continual CosineCRUST}\label{alg:cosineCRUST}
\begin{algorithmic}[1]
\State \textbf{Input}: Model $f$, Parameters $\theta$, Learning rate $\eta$, Layers $L$, Class $i$ dataset $V_i$, Input dataset ($x_t$, $y_t$), Initialized empty Coreset dictionary $S$, Minimum coreset size $A$, Phase 1 learning epochs $m$, Total Epochs $n$
\For{$i$ in \texttt{Experiences}}
    \For{epoch in $1, \dots, n$}
        \If{epoch in \{1, \ldots, m\}}
            \State $S[i]$ $\longleftarrow$ Total Class Data $V_i$ 
        \ElsIf{epoch in \{m+1, \ldots, n\}}
            \State \texttt{Forward pass:} $f(x_t, \theta)$
            \State $\mathcal{L} \longleftarrow l_{ce} (f(x_t, \theta), y_t)$
            \State $\nabla_S$ $\longleftarrow$ $\nabla(\mathcal{L}(f, f_{L-1}))$
            \State $k$ clusters $\gets \text{ClusterUsing}(\text{cos}_{\text{dist}}(\nabla_S))$
            \State $p \gets \{\text{Clusters} \mid \text{size(Cluster)} > A \}$
            \State $S[i]$ $\longleftarrow$ CRUST($p$ Clusters)
        \EndIf
        \For{($x_t$, $y_t$) in $S$}
            \State Forward $f(x_t, \theta)$
            \State $\mathcal{L} \longleftarrow l_{ce} (f(x_t, \theta), y_t)$
            \State \texttt{Total derivative:} $\nabla(\mathcal{L})$
            \State $\theta$ $\longleftarrow$ $\theta$ - $\eta$ * $\nabla(\mathcal{L})$
        \EndFor
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

